Revisiting Crowd Counting: State-of-the-art, Trends, and Future Perspectives

Crowd counting is an effective tool for situational awareness in public places. Automated crowd counting using images and videos is an interesting yet challenging problem that has gained significant attention in computer vision. Over the past few years, various deep learning methods have been developed to achieve state-of-the-art performance. The methods evolved over time vary in many aspects such as model architecture, input pipeline, learning paradigm, computational complexity, and accuracy gains etc. In this paper, we present a systematic and comprehensive review of the most significant contributions in the area of crowd counting. Although few surveys exist on the topic, our survey is most up-to date and different in several aspects. First, it provides a more meaningful categorization of the most significant contributions by model architectures, learning methods (i.e., loss functions), and evaluation methods (i.e., evaluation metrics). We chose prominent and distinct works and excluded similar works. We also sort the well-known crowd counting models by their performance over benchmark datasets. We believe that this survey can be a good resource for novice researchers to understand the progressive developments and contributions over time and the current state-of-the-art.

==> biographies/hamid.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hamid.jpg}}]{Hamid Menouar} (SM’16) is a Senior Research and Development Expert at Qatar Mobility Innovations Center (QMIC), Qatar, where he leads the development of innovations in the area of smart cities and smart living.  
Before moving to Qatar in 2010, Hamid worked for 8 years at Hitachi research lab in Sophia Antipolice, France, where he contributed and led research and development activities related to connected vehicles. During his experience with Hitachi, he has heavily contributed to the development of connected vehicles communication standards in Europe through an active participation at ETSI TC ITS and Car to Car Communication Consortium.  
Hamid received the Engineering degree (M.S.) in computer science from the University of Science and Technology Houari Boumediene, Algiers, Algeria, in 2003, the DEA (M.S.) degree in systems and information technologies from the University of Technology of Compiegne, France, 2004, and the Ph.D. degree in computer science from Telecom ParisTech, Paris, France, in 2008. 
\end{IEEEbiography}

==> biographies/hamila.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hamila.jpg}}]{Prof. Ridha Hamila} received the MSc, LicTech with distinction, and PhD degrees from Tampere University of Technology (TUT), Tampere, Finland, in 1996, 1999, and 2002, respectively. Dr. Hamila currently a Full Professor at the Department of Electrical Engineering, Qatar University, Qatar. From 1994 to 2002 he held various research and teaching positions at TUT within the Department of Information Technology, Finland. From 2002 to 2003 he was a System Specialist at Nokia research Center and Nokia Networks, Helsinki. From 2004 to 2009 he was with Emirates Telecommunications Corporation, UAE. Also, from 2004 to 2013 he was adjunct Professor at the Department of Communications Engineering, TUT. His current research interests include mobile and broadband wireless communication systems, Mobile Edge Computing, Internet of Everything, and Machine Learning. In these areas, he has published over 200 journal and conference papers most of them in the peered reviewed IEEE publications, filed seven US patents, and wrote numerous confidential industrial research reports.  Dr. Hamila has been involved in several past and current industrial projects, Ooreedo, Qatar National Research Fund, Finnish Academy projects, EU research and education programs. He supervised a large number of under/graduate students and postdoctoral fellows. He organized many international workshops and conferences. He is a Senior Member of IEEE.
\end{IEEEbiography}

==> biographies/khan.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biographies/khan.jpg}}]{Muhammad Asif Khan} (SM'20) received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{http://www.asifk.me}.
\end{IEEEbiography}


%% Other journals using picinpar package
% \parpic{\includegraphics[width=1in,clip,keepaspectratio]{biographies/khan.jpg}}
% \noindent {\bf Muhammad Asif Khan} received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET.
% % For more detailed information, please visit his homepage: \url{http://www.asifk.me}.

% \authorbiography[scale=0.3,overhang=0pt,wraplines=9,imagewidth=3cm,imagepos=]{biographies/khan.jpg}{Muhammad Asif Khan}
% {received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{http://www.asifk.me}}


==> figures/fig_cc_methods.tex <==



\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/PDFs/cc_methods.pdf}
    \caption{Crowd counting methods: total count regression (top), versus density map estimation (bottom)}
    \label{fig:cc_methods}
\end{figure}

==> other_tex/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tables/tab_crowd_mon_areas.tex <==
\begin{table*}[htbp] 
\caption{Areas of Crowd Monitoring.}
\label{tab:crowd_mon_areas}
% \rmfamily % \sffamily sans-serif \rmfamily roman \ttfamily typewriter
\centering
\begin{tabular}{llrl}
\toprule
\bfseries Area &\bfseries Topics &\bfseries Reference Studies &\bfseries Description of Study \\ \midrule 
% \cmidrule(lr){1-1}  \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}

%===========================================
%    Counting
%===========================================
\multirow{2}{*}{Crowd Counting} &\multirow{2}{*}{Counting objects}
&[X][X] &Counting people in CCTV footage. \\[0.5em]
& &\cite{arteta2016} &Counting penguins in the wild using aerial images. 
\\[1em]
% \hline \hline


\multirow{2}{*}{Localization}  &\multirow{2}{*}{Localization}
&[X][X] &Study 1 \\[0.5em]
& &[X][X] &Study 2
\\[1em]
% \hline \hline


\multirow{2}{*}{Motion Analysis}  &\multirow{2}{*}{Object tracking}
&[X][X] &Study 1  \\[0.5em]
& &[X][X] &Study 2
\\[1em]
% \hline \hline


\multirow{2}{*}{Behavior Recognition}  &\multirow{2}{*}{Crowd Behavior}
&[X][X] &Study 1 \\[0.5em]
& &[X][X] &Study 2
\\[1em]

&\multirow{2}{*}{Individual Behavior}
&[X][X] &Study 1 \\[0.5em]
& &[X][X] &Study 2 \\[0.5em]


\bottomrule
\end{tabular}
\end{table*}

==> tables/tab_model_complexity.tex <==


\begin{table}[]
\centering
\renewcommand*{\arraystretch}{1.5}
\caption{Comparison of crowd counting models for number of parameters (in Million), GMACs, size (in MB), and inference time (in seconds). The input size is kept fixed as $400\times400.$}
\label{tab:model_complexity}
\begin{tabular}{ccccc} \toprule
Model    &Parameters  &Size   &GMACs &Inference Time  \\[0.2em] \midrule
CrowdCNN \cite{CrowdCNN_CVPR2015}    & &  & & \\ 
MCNN \cite{MCNN_ICIP2017}    &0.13 &0.53 &4.31   & \\
CMTL  \cite{CMTL_AVSS2017}    &  & & & \\ 
CSRNet \cite{CSRNet_CVPR2018}    &16.26 &65.05  &66.13 & \\
SANet \cite{SANet_ECCV2018}    &0.91 &3.64  & & \\
RTCNN (ours)   &  & & \\ \bottomrule
\end{tabular}
\end{table}

==> tables/tab_surveys.tex <==
\begin{table*}[htbp]
\caption{Existing Studies on Crowd Monitoring}
\label{tab:crowd_mon_surveys}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Ref &Year &Category &Topics Covered &Topics not Covered \\ \hline \hline
\cite{akbar2020} &2020 &Crowd Monitoring &Localization, Datasets &Crowd Counting, Behavior
Analysis \\[0.5em]
\cite{gao2020} &2020 &Crowd Counting &Counting, density estimation &ABC \\[0.5em]



\hline
\end{tabular}
\end{table*}
